6IMPOSE: Bridging the Reality Gap in 6D Pose Estimation for Robotic Grasping

6D pose recognition has been a crucial factor in the success of robotic grasping, and recent deep learning based approaches have achieved remarkable results on benchmarks. However, their generalization capabilities in real-world applications remain unclear. To overcome this gap, we introduce 6IMPOSE, a novel framework for sim-to-real data generation and 6D pose estimation. 6IMPOSE consists of four modules: First, a data generation pipeline that employs the 3D software suite Blender to create synthetic RGBD image datasets with 6D pose annotations. Second, an annotated RGBD dataset of five household objects generated using the proposed pipeline. Third, a real-time two-stage 6D pose estimation approach that integrates the object detector YOLO-V4 and a streamlined, real-time version of the 6D pose estimation algorithm PVN3D optimized for time-sensitive robotics applications. Fourth, a codebase designed to facilitate the integration of the vision system into a robotic grasping experiment. Our approach demonstrates the efficient generation of large amounts of photo-realistic RGBD images and the successful transfer of the trained inference model to robotic grasping experiments, achieving an overall success rate of 87% in grasping five different household objects from cluttered backgrounds under varying lighting conditions. This is made possible by the fine-tuning of data generation and domain randomization techniques, and the optimization of the inference pipeline, overcoming the generalization and performance shortcomings of the original PVN3D algorithm. Finally, we make the code, synthetic dataset, and all the pretrained models available on Github.

==> sections/figures.tex <==
\newpage
\section*{Figures}

\begin{figure}[h!]
\begin{center}
\includegraphics[width=\linewidth]{images/diagram.jpg}% This is a *.eps file
\end{center}
\caption{A two-stage pose estimation approach showing the object detection with YOLO-tiny to localize the object of interest at the first stage, followed by the 6D object pose estimation with PVN3D-tiny at the second stage.}\label{fig:two-stages}
\end{figure}

\begin{subfigure}
\begin{center}
    \begin{minipage}[b]{0.9\columnwidth}
        \centering
        \includegraphics[width=0.3\columnwidth]{images/lm_cat_rgb.png}
        \includegraphics[width=0.3\columnwidth]{images/lm_cat_depth.png} 
        \includegraphics[width=0.3\columnwidth]{images/lm_cat_normals.png}
        \caption{Real data}
        \label{fig:real}
    \end{minipage}  

    \begin{minipage}[b]{0.9\columnwidth}
        \centering
        \includegraphics[width=0.3\columnwidth]{images/bl_cat_rgb.png} 
        \includegraphics[width=0.3\columnwidth]{images/bl_cat_depth.png} 
        \includegraphics[width=0.3\columnwidth]{images/bl_cat_normals.png}
        \caption{Rendered data}
        \label{fig:render}
    \end{minipage}

    \begin{minipage}[b]{0.9\columnwidth}
        \centering
        \includegraphics[width=0.3\columnwidth]{images/bl_cat_rgb_aug.png} 
        \includegraphics[width=0.3\columnwidth]{images/bl_cat_depth_aug.png} 
        \includegraphics[width=0.3\columnwidth]{images/bl_cat_normals_aug.png}
        \caption{Augmented data}
        \label{fig:aug}
    \end{minipage}

\setcounter{subfigure}{-1}
    \caption{The figure showing the visualization of RGB images (Left), depth images (Middle) and surface normals (Right) for real data \textbf{(a)}, rendered synthetic data \textbf{(b)} and augmented synthetic data \textbf{(c)}.}
    \label{fig:real-synthetic}
\end{center}
\end{subfigure}

\begin{figure}[h!]
    \begin{center}
    \includegraphics[width=0.6\columnwidth]{images/psd.pdf}
    \end{center}
    \caption{The plot showing the qualitative average power spectral density (PSD) of depth images with respect to frequencies for the object ``cat" from LM dataset over 50 randomly sampled images.}
    \label{fig:psd}
\end{figure}

\begin{figure}[h!]
    \begin{center}
    \includegraphics[width=0.6\columnwidth]{images/duck_grasps.png}
    \end{center}
    \caption{The figure showing the automatically generated grasp poses for the household object ``duck" .}
    \label{fig:duck_grasps}
\end{figure}

% GRASPING FIGURE


\begin{figure}[h!]
\begin{center}
    \begin{minipage}[b]{0.9\columnwidth}
    \centering
    \includegraphics[width=0.3\columnwidth]{images/objects_camera.jpg}
    \includegraphics[width=0.3\columnwidth]{images/objects_rgb.png} 
    \includegraphics[width=0.3\columnwidth]{images/objects_depth.png}
    \end{minipage} 
    \caption{The figure showing the photographed \textbf{(left)}, photo-realistically rendered RGB \textbf{(middle)} and rendered depth images \textbf{(right)} for the five selected household objects.}
    \label{fig:five_objects}
\end{center}
\end{figure}

\begin{subfigure}
\begin{center}
    \begin{minipage}[b]{\columnwidth}
    \centering
    \includegraphics[width=0.24\columnwidth]{images/normal_lighting_square.jpg}
    \includegraphics[width=0.24\columnwidth]{images/normal_camera_rgb.png} 
    \includegraphics[width=0.24\columnwidth]{images/normal_camera_depth.png}
    \includegraphics[width=0.24\columnwidth]{images/normal_rgb_pose.png}
    \caption{Experiments under diffused lighting condition.}
    \label{fig:exp_normal}
    \end{minipage}  

    \begin{minipage}[b]{\columnwidth}
    \centering
    \includegraphics[width=0.24\columnwidth]{images/dark_lighting_square.jpg}
    \includegraphics[width=0.24\columnwidth]{images/low_camera_rgb.png} 
    \includegraphics[width=0.24\columnwidth]{images/low_camera_depth.png}
    \includegraphics[width=0.24\columnwidth]{images/low_rgb_pose.png}
    \caption{Experiments under low lighting condition.}
    \label{fig:exp_low}
    \end{minipage}  
    
    \begin{minipage}[b]{\columnwidth}
    \centering
    \includegraphics[width=0.24\columnwidth]{images/biased_lighting_square.jpg}
    \includegraphics[width=0.24\columnwidth]{images/biased_camera_rgb.png} 
    \includegraphics[width=0.24\columnwidth]{images/biased_camera_depth.png}
    \includegraphics[width=0.24\columnwidth]{images/biased_rgb_pose.png}
    \caption{Experiments under spot lighting condition.}
    \label{fig:exp_spot}
    \end{minipage}  
    
    \setcounter{subfigure}{-1}
    \caption{The figure showing the real world grasping experiments under diffused \textbf{(a)}, low \textbf{(b)}, spot \textbf{(c)} lighting conditions. The experimental setup, RGB view, depth view and the predicted pose of pliers on RGB are shown from the left to the right.}
    
\label{fig:real-grasp}
\end{center}
\end{subfigure}




==> sections/related_work.tex <==
\section{Related Work}
In this section, we review state-of-the-art data-driven 6D pose estimation algorithms using RGBD images. We also compare the current training data preparation techniques.

\subsection{6D pose estimation from RGBD}

Estimating 6D poses from a single RGB image is challenging due to many factors. First, the learning algorithms suffer from perspective ambiguities, where the appearances of the objects are similar under different viewpoints. Such a problem is further exacerbated when objects are highly occluded\cite{zakharov2019dpod}. Second, like in many computer vision tasks, the performance of the algorithms is vulnerable to environmental factors, such as lighting variations and cluttered background \cite{peng2019pvnet}. The challenges are recently eased by using depth images, where the geometry information is presented. 

One way to leverage depth images is to use depth information to refine the poses predicted from RGB images \cite{sundermeyer2018implicit} \cite{kehl2017ssd}. \cite{sundermeyer2018implicit} leverages an Augmented autoencoder to reconstruct the object from the input image. Then the initial pose is determined by selecting the highest \textit{cos} similarity between the reconstructed image and the code from a predefined codebook. \cite{kehl2017ssd} treat the pose estimation as a classification problem and leverage the SSD \cite{liu2016ssd} to output the pose directly. In these two algorithms\cite{sundermeyer2018implicit}\cite{kehl2017ssd}, the depth can be optionally used to refine the initial pose with the Iterative Closest Point algorithm (ICP).

Another direction is to direct infer 6D Pose from the point cloud \cite{chen2020g2l}\cite{hagelskjaer2021bridging}. In this case, the object detection network or segmentation network first localizes the target object to get the point cloud of interest, on which the point cloud network finishes the 6D pose prediction. \cite{chen2020g2l} first use RGB to globally localize the object and segment the point cloud of the object from the background. Then a point cloud network is directly working on the segmented point cloud to predict the pose. Similarly, \cite{hagelskjaer2021bridging} use Mask RCNN \cite{he2017mask} to first select the point cloud and use modified DGCNN \cite{wang2019dynamic} to directly work on the point cloud to predict the pose.

The depth image can also be used to provide complementary geometry information along with appearance information provided from RGB to have better representation learning \cite{xu2018pointfusion} \cite{li2018unified} \cite{wang2019densefusion} \cite{he2020pvn3d} \cite{he2021ffb6d}\cite{lin2022e2ek}. To this end, the depth information is first converted to a point cloud, where the deep geometry features are extracted with a point cloud network. As for RGB inputs, the appearance deep features are extracted with a RGB network. The extracted deep features can be fused in two different ways. \cite{xu2018pointfusion} \cite{li2018unified} simply concatenated the deep RGB features to deep depth features. \cite{wang2019densefusion} \cite{he2020pvn3d} fuse the deep features at the pixel level. \cite{he2021ffb6d} further explores the bidirectional features fusion at different stages of representation learning. Followingly, \cite{lin2022e2ek} develops a two-stage approach by leveraging YOLO-V3 \cite{redmon2018yolov3} and FFBf6D \cite{he2021ffb6d} to have better performance. 

\subsection{Training data augmentation}
The training of 6D pose estimation deep models is non-trivial and usually imposes huge demand of training data \cite{kaskman2019homebreweddb}. In 6D pose estimation domain, some public datasets are available, like LineMod \cite{hinterstoisser2012model} and YCB \cite{xiang2018posecnn}. Meanwhile a few domain-specific dataset like \cite{kaskman2019homebreweddb} \cite{kleeberger2019large} are also proposed for robotic grasping applications. However, the images provided in these datasets are typically not sufficient for training complex 6D pose estimation deep neural networks \cite{xiang2018posecnn}. Thus, many algorithms need to use augmented dataset for training \cite{sundermeyer2018implicit} \cite{kehl2017ssd} \cite{he2020pvn3d} \cite{he2021ffb6d} \cite{hagelskjaer2021bridging} 

Nowadays, modern simulations, such as Unity, Blender, OpenGL enables high-quality realistic rendering. And these simulations are often used to generate synthetic data to expand the training dataset. \cite{sundermeyer2018implicit} and \cite{kehl2017ssd} render 3D meshes in OpenGL to get RGB images with random background from commonly used computer vision dataset, for example Pascal VOC\cite{everingham2012pascal}, MS COCO \cite{lin2014microsoft}. \cite{he2020pvn3d} \cite{lin2022e2ek} \cite{he2021ffb6d} \cite{wang2019densefusion} use the synthetic generated from \cite{xiang2018posecnn}, where the datapoint is generated by rendering 3D meshes in Z-buffer \cite{} with sampled poses. \cite{hagelskjaer2021bridging} leverages the data generated from Blender \cite{blender}. Recently, Unity \cite{borkman2021unity} also supports RGBD simuations. 

However, after training on the synthetic data, the performance of the learned 6D pose estimation algorithm deteriorates when tested on the real images \cite{sundermeyer2018implicit} \cite{xiang2018posecnn}.  To mitigate the gap between simulated and real images, many works apply domain randomization \cite{Tobin2017domainrandomization} on the synthetic data. The domination randomization usually lies in two main aspects. The first aspect is to randomize the scene, where the pose of objects, backgrounds and some environmental variables such as lightness are randomized to cover as many scenarios as possible \cite{sundermeyer2018implicit}\cite{hagelskjaer2021bridging}\cite{liu2016ssd}. And another aspect is to randomize the properties of the RGB and Depth images. For RGB images, the randomization focuses on changing image contrast, brightness, Gaussian blur color distortion \cite{sundermeyer2018implicit} \cite{kehl2017ssd}. As for depth images, the depth frequency is important, which is often randomized by injecting Gaussin and Perlin Noise \cite{thalhammer2019sydpose}.




==> sections/tables.tex <==
\newpage
\section*{Tables}
\begin{table*}[htbp]
\caption{The performance of 6D pose estimation on LineMOD compares to the state-of-the-art using RGBD. The bold objects are symmetric.}
\begin{center}
\resizebox{\linewidth}{!}{
{\small{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
\toprule[1.5pt]
 &\multicolumn{6}{c|}{\textbf{Real data}} &\multicolumn{4}{c}{\textbf{Synthetic Data}} \\
\cline{2-11} 
 & \textbf{PointFusion$^1$}
 & \textbf{DenseFusion$^2$$^{\mathrm{*}}$}
 & \textbf{G2L-Net$^3$}
 & \textbf{PVN3D$^4$}
 & \textbf{FFB6D$^5$}
 & \textbf{E2EK$^6$}
 & \textbf{AAE$^7$$^{\mathrm{*}}$}
 & \textbf{SSD-6D$^8$$^{\mathrm{*}}$}
 & \textbf{DGCNN$^9$$^{\mathrm{*}}$}
 & \textbf{Ours}  \\

 % & \textbf{\cite{xu2018pointfusion}}
 % & \textbf{\cite{wang2019densefusion}}
 % & \textbf{\cite{chen2020g2l}}
 % & \textbf{\cite{he2020pvn3d}}
 % & \textbf{\cite{he2021ffb6d}}
 % & \textbf{\cite{lin2022e2ek}} 
 % & \textbf{\cite{sundermeyer2018implicit}}  
 % & \textbf{\cite{kehl2017ssd}} 
 % & \textbf{\cite{hagelskjaer2021bridging}} 
 % &   \\
\midrule[1.1pt]
Ape  &70.4 &92.3 &96.8 &97.3 &98.4 &98.7 &20.55 & 65 & 97.7 & 78 \\
Benchvise  &80.7 &93.2 &96.1 &99.7 &100 &100 &64.25 & 80 & 99.8 & 92   \\
Camera  &60.8 &94.4 &98.2 &99.6 &99.9 &99.9 &63.20 & 78 & 98.3 & 66 \\
Can  &61.1 &93.1 &98 &99.5 &99.8 &100 &76.09 & 86 & 98.8 & 95 \\
Cat  &79.1 &96.5 &99.2 &99.8 &99.9 &100 &72.01 & 70 & 99.9 & 97 \\
Driller &47.3 &87 &99.8 &99.3 &100 &100 &41.58 & 73 & 99.2 & 91  \\
Duck  &63 &92.3 &97.7 &98.2 &98.4 &99.4 & 32.38 & 66 & 97.8 & 89 \\ 
\textbf{Eggbox} &99.9 &99.8 &100 &99.8 &100 & 100& 98.64 & 100 & 97.7 & 91 \\
\textbf{Glue} &99.3 &100 &100 &100 &100 &100 &96.39 & 100 & 98.9 & 73 \\
Holepuncher  &71.8 &92.1 &99 &99.9 &99.8 &100 & 49.88 &  49 & 94.1 & 61 \\
Iron &83.2 &97 &99.3 &99.7 &99.9 &100 & 63.11 & 78 & 100 & 94  \\
Lamp &62.3 &95.3 &99.5 &99.8 &99.9 &99.9 & 91.69 & 73 & 92.8 & 87 \\
Phone &78.8 &92.8 &98.9 &99.5 &99.7 & 100 & 70.96 & 79 & 99.1 & 74 \\
\midrule[1.1pt]
All &73.7& 94.3 &98.7& 99.4& 99.7& 99.8& 64.67 & 79 & 98.0 & 83.6 \\
\midrule[1.1pt]
\textbf{Speed(s)} & \cancel{}{} & 0.06 & 0.044 & 0.19  &0.075 & 0.068 & \cancel{} & 0.1 &1.0 & 0.046\\
\bottomrule[1.5pt]
\multicolumn{4}{l}{$^{\mathrm{*}}$ With refinement} \\
\multicolumn{11}{l}{$^1$\cite{xu2018pointfusion}; $^2$\cite{wang2019densefusion}; $^3$\cite{chen2020g2l}; $^4$\cite{he2020pvn3d}; $^5$\cite{he2021ffb6d}; $^6$\cite{lin2022e2ek} $^7$\cite{sundermeyer2018implicit};} \\
\multicolumn{11}{l}{$^8$\cite{kehl2017ssd}; $^9$\cite{hagelskjaer2021bridging}} \\


\end{tabular}
}}}
\label{tab: LineMOD_evaluation}
\end{center}
\end{table*}

\begin{table*}[htbp]
\caption{6D pose estimation ADD(S) scores, using predicted or ground truth bounding boxes}
\begin{center}
\resizebox{\columnwidth}{!}{
{\small{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule[1.5pt]
 & Ape & Benchvise & Camera & Can & Cat & Driller & Duck & \textbf{Eggbox} & \textbf{Glue} & Holepuncher & Iron & Lamp & Phone & All \\
\midrule[1.1pt]
Predicted bboxes & 78 & 92 & 66 & 95 & 97 & 91 & 89 & 91 & 73 & 61 & 94 & 87 & 74 & 83.6 \\
GT bboxes & 81 & 99 & 98 & 96 & 97 & 99 & 94 & 99 & 99 & 78 & 96 & 94 & 96 & 94.3 \\
\bottomrule[1.5pt]
\end{tabular}
}}}
\label{tab:LineMOD_ablat}
\end{center}
\end{table*}

\begin{table}[htbp]
\caption{Running time analysis of the proposed two-stage pose estimation approach}
\begin{center}
\resizebox{0.6\columnwidth}{!}{
{\small{
\begin{tabular}{c|c|c}
\toprule[1.5pt]
Procedures & Speed Mean/Std(ms) & Percent\\
\midrule[1.1pt]
YOLO-V4 tiny & 6.7/0.5 & 15\% \\
Pcld preproc. & 8.2/5.9 & 18\% \\
PVN3D tiny & 23.7/0.9 & 51\% \\
Pose regression  & 7.2/0.7 & 16\% \\
\midrule[1.1pt]
All & 45.8/6.2 & 100\% \\
\bottomrule[1.5pt]
\end{tabular}
}}}
\label{time_analysis}
\end{center}
\end{table}



\begin{table}[htbp]
\caption{Single Object grasping experiments under variable lighting conditions}
\begin{center}
\resizebox{\columnwidth}{!}{
{\small{
\begin{tabular}{c|ccccccc}
\toprule[1.5pt]
Conditions                                         & \multicolumn{1}{c|}{Category}     & \multicolumn{1}{c|}{Duck}   & \multicolumn{1}{c|}{Stapler} & \multicolumn{1}{c|}{Glue}   & \multicolumn{1}{c|}{Chewtoy$^{\mathrm{*}}$} & \multicolumn{1}{c|}{Pliers} & \textbf{All}                        \\ 
\midrule[1.1pt]
\multirow{5}{*}{Diffused}                          & \multicolumn{1}{c|}{Success}      & \multicolumn{1}{c|}{47}     & \multicolumn{1}{c|}{46}      & \multicolumn{1}{c|}{46}     & \multicolumn{1}{c|}{45}      & \multicolumn{1}{c|}{40}     & 224                                 \\
                                                   & \multicolumn{1}{c|}{Grasp missed} & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{3}       & \multicolumn{1}{c|}{4}      & \multicolumn{1}{c|}{1}       & \multicolumn{1}{c|}{5}      & 15                                  \\
                                                   & \multicolumn{1}{c|}{Collision}    & \multicolumn{1}{c|}{1}      & \multicolumn{1}{c|}{1}       & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{4}       & \multicolumn{1}{c|}{5}      & 11                                  \\ 
                                                   & \multicolumn{1}{c|}{SR} & \multicolumn{1}{c|}{94.0\%} & \multicolumn{1}{c|}{92.0\%}  & \multicolumn{1}{c|}{92.0\%} & \multicolumn{1}{c|}{90.0\%}  & \multicolumn{1}{c|}{80.0\%} & \multicolumn{1}{c}{\textbf{89.6\%}} \\
                                                   & \multicolumn{1}{c|}{SR w.o collision} & \multicolumn{1}{c|}{95.9\%} & \multicolumn{1}{c|}{93.9\%}  & \multicolumn{1}{c|}{92.0\%} & \multicolumn{1}{c|}{97.8\%}  & \multicolumn{1}{c|}{88.9\%} & \multicolumn{1}{c}{\textbf{93.7\%}} \\ \midrule[1.0pt]
\multirow{5}{*}{Low}                               & \multicolumn{1}{c|}{SR}      & \multicolumn{1}{c|}{47}     & \multicolumn{1}{c|}{38}      & \multicolumn{1}{c|}{43}     & \multicolumn{1}{c|}{42}      & \multicolumn{1}{c|}{41}     & 211                                 \\
                                                   & \multicolumn{1}{c|}{Grasp missed} & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{8}       & \multicolumn{1}{c|}{4}      & \multicolumn{1}{c|}{2}       & \multicolumn{1}{c|}{7}      & 24                                  \\
                                                   & \multicolumn{1}{c|}{Collision}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{4}       & \multicolumn{1}{c|}{3}      & \multicolumn{1}{c|}{6}       & \multicolumn{1}{c|}{2}      & 15                                  \\ 
                                                   & \multicolumn{1}{c|}{SR} & \multicolumn{1}{c|}{94.0\%} & \multicolumn{1}{c|}{76.0\%}  & \multicolumn{1}{c|}{86.0\%} & \multicolumn{1}{c|}{84.0\%}  & \multicolumn{1}{c|}{82.0\%} & \textbf{84.4\%}  \\
                                                   & \multicolumn{1}{c|}{SR w.o collision} & \multicolumn{1}{c|}{94.0\%} & \multicolumn{1}{c|}{82.6\%}  & \multicolumn{1}{c|}{91.5\%} & \multicolumn{1}{c|}{95.5\%}  & \multicolumn{1}{c|}{85.4\%} & \textbf{89.8\%}                     \\ \midrule[1.0pt]
\multirow{5}{*}{Spot}                              & \multicolumn{1}{c|}{Success}      & \multicolumn{1}{c|}{48}     & \multicolumn{1}{c|}{43}      & \multicolumn{1}{c|}{44}     & \multicolumn{1}{c|}{39}      & \multicolumn{1}{c|}{44}     & 218                                 \\
                                                   & \multicolumn{1}{c|}{Grasp missed} & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{2}       & \multicolumn{1}{c|}{2}      & \multicolumn{1}{c|}{1}       & \multicolumn{1}{c|}{3}      & 10                                  \\
                                                   & \multicolumn{1}{c|}{Collision}    & \multicolumn{1}{c|}{0}      & \multicolumn{1}{c|}{5}       & \multicolumn{1}{c|}{4}      & \multicolumn{1}{c|}{10}      & \multicolumn{1}{c|}{3}      & 22                                  \\  
                                                   & \multicolumn{1}{c|}{SR} & \multicolumn{1}{c|}{96.0\%} & \multicolumn{1}{c|}{86.0\%}  & \multicolumn{1}{c|}{88.0\%} & \multicolumn{1}{c|}{78.0\%}  & \multicolumn{1}{c|}{88.0\%} & \textbf{87.2\%}\\
                                                 & \multicolumn{1}{c|}{SR w.o collision} & \multicolumn{1}{c|}{96.0\%} & \multicolumn{1}{c|}{95.6\%}  & \multicolumn{1}{c|}{95.7\%} & \multicolumn{1}{c|}{97.5\%}  & \multicolumn{1}{c|}{93.6\%} & \textbf{95.6\%} \\   
                                                   
\midrule[1.1pt]
%\multicolumn{1}{l|}{\textbf{Overall success rate}} & \multicolumn{7}{c}{\textbf{87.06\%}}                                                                                                                                                                                            \\ \hline
\multirow{2}{*}{All conditions}                 & \multicolumn{1}{c|}{SR} & \multicolumn{1}{c|}{94.7\%} & \multicolumn{1}{c|}{84.7\%}  & \multicolumn{1}{c|}{88.7\%} & \multicolumn{1}{c|}{84.0\%}  & \multicolumn{1}{c|}{83.3\%} & \textbf{87.06\%}  \\
                                                & \multicolumn{1}{c|}{SR w.o collision} & \multicolumn{1}{c|}{95.3\%} & \multicolumn{1}{c|}{90.7\%}  & \multicolumn{1}{c|}{93.0\%} & \multicolumn{1}{c|}{96.9\%}  & \multicolumn{1}{c|}{89.3\%} & \textbf{93\%}  \\
\bottomrule[1.5pt]

\multicolumn{4}{l}{$^{\mathrm{*}}$ symmetrical object}
\end{tabular}
}}}
\label{grasp-exp}
\end{center}
\end{table}
